Towards Learning (Dis)-Similarity of Source Code from Program Contrasts

Understanding the functional (dis)-similarity of source code is significant for code modeling tasks such as software vulnerability and code clone detection. We present DISCO(DIS-similarity of COde), a novel self-supervised model focusing on identifying (dis)similar functionalities of source code. Different from existing works, our approach does not require a huge amount of randomly collected datasets. Rather, we design structure-guided code transformation algorithms to generate synthetic code clones and inject real-world security bugs, augmenting the collected datasets in a targeted way. We propose to pre-train the Transformer model with such automatically generated program contrasts to better identify similar code in the wild and differentiate vulnerable programs from benign ones. To better capture the structural features of source code, we propose a new cloze objective to encode the local tree-based context (e.g., parents or sibling nodes). We pre-train our model with a much smaller dataset, the size of which is only 5% of the state-of-the-art models' training datasets, to illustrate the effectiveness of our data augmentation and the pre-training approach. The evaluation shows that, even with much less data, DISCO can still outperform the state-of-the-art models in vulnerability and code clone detection tasks.

==> acl2022/body/10_reproducibility_stmt.tex <==
% We are 

==> acl2022/body/1_intro.bck.tex <==
\section{Introduction}
\label{sec1:intro}

%  HOw many paragraphs? 

Large pre-trained models have been applied for source code and reported promising performance for code understanding\brc{generation also requires understanding} and generation tasks. Pre-training with enormous amount of open-source programs, existing techniques have successfully captured the textual code features using token-based tasks~\citep{feng2020codebert, buratti2020cbert, cubert}, such as masked language model and next sentence prediction. Some works further explored the potentials of leveraging structural characteristics of programming languages to understand code~\citep{guo2021graphcodebert, Jiang2021TreeBERT}. 
% While these approaches demonstrate good understanding about code tokens and structures, 
However, even with good understanding about code tokens and structures, the model can still get confused when trying to differentiate code functionalities. 
Two programs can have different tokens and structures while achieving the same functionality, \ie semantic clones. On the other hand, two programs that share the syntax and most of the tokens can have significantly distinct behaviors. For instance, if we just replace $<$ with $\leq$ of a boundary checking statement before accessing an array, the program's functionality 
% can be unpredictable and even trigger security issues
can trigger severe security vulnerability \eg buffer overflow bug\footnote{https://en.wikipedia.org/wiki/Buffer\_overflow}. 
%\scc{The following line does not really go with the current paragraph context. } 
Existing pretraining technique does not learn anyth\brc{incomplete senctence}
In addition, existing pre-training techniques always require really large datasets and expensive hardware to achieve promising performance for downstream tasks. For developers and researchers who have limited access to large datasets and premium equipment, it is challenging to explore such source code pre-training 
% as per their requests
.

In this work, we present \tool, a self-supervised pre-trained model that jointly learn the textual, syntactic and functional properties of source code. 
% To capture 
To learn about the structural properties of code, we propose a new pre-training task, \emph{node-type masked language model (NT-MLM)}, which can embed the local tree-based contexts together with the token-based contexts into each token. 

\scc{Review this}To deal with the limitation of existing pre-training techniques, we intentionally train the model to recognize similar programs and differentiate buggy programs with the benign ones, not only based on their textual and syntactic code similarity. 
However, collecting a human-labeled dataset that has both functionally equivalent and bug/patch code pairs and contains enough data for model pre-training is very difficult and time-consuming, so we design structure-guided code transformation heuristics to automatically augment the training sample with one positive and one hard negative contrasts. The positive contrast will be functionally equivalent to the original code while look quite different. The negative contrast is textually and syntactically very similar code but enclosed with bugs and security issues. We apply contrastive learning to bring the functionally similar code embeddings closer and separate the buggy programs further from the benign ones in the vector space. 

%In this work, we present \tool, a self-supervised pre-trained model that jointly learn the textual, syntactic and functional properties of source code. To better capture the functionality of programs, we design structure-guided code transformation heuristics to augment the training data \emph{without human labels}. For each sample, we generate 1) functionally equivalent code that looks different from the original one, and 2) textually and syntactically very similar code but enclosed with bugs and security issues. Having these pairs, we apply \emph{contrastive learning} and train the model to recognize similar programs and differentiate buggy programs with the benign ones, not only based on their textual and syntactic code similarity. We further propose a new pre-training task, \emph{node-type masked language model (NT-MLM)}, which can embed the local tree-based contexts together with the token-based contexts into each token.

% We collect our pre-training corpus from the most popular open-source C and Java projects and end up with 865 MB C code and 992MB Java code.

We carefully designed \tool's  pre-training to learn about syntactic and functional relationship between code components and we expect \tool to learn sufficient knowledge for downstream applications from limited amount of data, consequently saving computing resources.
% With the complicated and carefully design of our pre-training, we expect \tool to learn sufficient knowledge for downstream applications from limited amount of data and consequently save computing resources. 
To this end, we pre-train \tool on a \emph{small} dataset, with 865 MB of C code and 992 MB Java code from 100 most popular GitHub, and evaluate the model on code understanding and generation tasks: vulnerability detection, code clone detection and code summarization. Experiments show that our small models can outperform many baselines that are pre-trained on much larger datasets. Our analysis further illustrates that by adding hard negative code samples and the new NT-MLM objective, the model can better understand code during pre-training. The ablation study also reveals the potentials of pre-training our model with larger datasets and further improve the performance.

In summary, our major contributions are: 1) We design structure-guided code transformation heuristics to augment training data without human labels. We introduce \emph{hard negative code samples} for the first time, to better learn code contrasts. Our automated bug injection strategy successfully encloses real-world security issues to the code. 2) We propose a new pre-training task, NT-MLM, to embed structural context to each token embedding. 3) We develop \tool, a self-supervised pre-training technique that can jointly and efficiently learn the textual, syntactic and functional properties of code. Even though pre-trained with significantly less data, \tool can match or outperform the state-of-the-art models on code understanding and generation tasks.


==> acl2022/body/1_intro_bck_bck.tex <==
\section{Introduction}
\label{sec1:intro}

%  HOw many paragraphs? 

Large pre-trained models have been applied for source code and reported promising performance for code understanding and generation tasks. 
These models have successfully captured the code features by treating code as text sequences~\citep{feng2020codebert, buratti2020cbert, cubert}.
%These models have successfully captured the textual code features using token-based tasks~\citep{feng2020codebert, buratti2020cbert, cubert}, such as masked language model and next sentence prediction. 
Some works further explored the potentials of leveraging structural characteristics of programming languages (\eg abstract syntax tree and code graph) to understand code~\citep{guo2021graphcodebert, Jiang2021TreeBERT}. 

However, even with a good understanding of code syntax (\ie tokens and structures), 
such pre-trained models can get confused when understanding code functionalities. 
For instance, two code fragments having identical functionality (a.k.a. semantic clones) but different syntax may not be recognized as similar by the existing models. 
Likewise, these models cannot distinguish between two code fragments that differ in functionalities but share close syntactic resemblance. For example, consider an if statement {\tt if(len(buf) $<$ N)} checking buffer length before accessing the buffer. Keeping the rest of the program the same, if we simply replace the token `$<$' with `$\leq$', the modification can potentially trigger security vulnerability \eg buffer overflow bug\footnote{https://en.wikipedia.org/wiki/Buffer\_overflow}. It is challenging for existing pre-training techniques to capture such subtle differences in the functionalities.

%Existing pre-training techniques cannot capture such subtle differences in the functionalities. 
% In addition, existing pre-training techniques always require large datasets and expensive hardware to achieve promising performance for downstream tasks. It is challenging for developers and researchers who have limited access to large datasets and premium equipment to explore such largescale source code pretraining.

To address these limitations,  we present \tool, a self-supervised pre-trained model that jointly learns code tokens, structures and functionalities.
%textual, syntactic, and functional properties of source code. 
For understanding code tokens, we use a standard masked language model (MLM).
To learn about the structural code properties, we propose a new pre-training task, \emph{node-type masked language model (NT-MLM)}, which can embed the local tree-based contexts together with the token-based contexts into each token.
Finally, to capture functional properties, we carefully design the pre-training to recognize the structurally different yet functionally identical programs (\ie positive samples) as similar and to differentiate between structurally close but functionally different programs (\ie negative samples). We apply contrastive learning to bring the functionally similar code embeddings closer in the vector space and vice versa. 

However, collecting a human-annotated dataset having both positive and negative samples, especially at the scale of for  usual pre-training, is difficult and time-consuming. To automate, we design structure-guided code transformation heuristics to automatically augment the training sample with one positive and one hard negative contrasts. 
The positive contrast will be functionally equivalent to the original code while look quite different. The negative contrast is textually and syntactically very similar but not the functionally identical code and likely to contain bugs and security issues. Using contrastive learning, we aim to place all the functionally similar code embeddings closer and separate the buggy programs further from the benign ones in the vector space.

Additional benefit of such carefully designed positive and negative sample generation is that we augment the data in a targeted manner.  In contrast, existing pretraining techniques rely on huge volume of training corpus, all are randomly selected. Given the main motivation of pretraining is to understand program's functionality~\citep{ahmad2021plbart}, such random selection of training data are not tailored for explicitly learning the functionalities. In contrast, 
our approach in learning such is through contrastive reasoning. Since the model {\em explicitly} learns to reason about a code \wrt its functional equivalent and different counterparts during pretraining, our pretrained model outperforms other models even with a much smaller pretrained dataset.

%\scc{additional benefit of our data processing.}
% Additional benefit of such carefully designed positive and negative sample generation is that we augment the data in a targeted manner. 
% Given understanding a program's functionality is the primary motivation for a pretraining model~\citep{ahmad2021plbart}, existing  techniques rely on randomly selecting 
% %aim at learning to reason about code behavior from 
% large corpora of source code, and thus, the methods are not tailored for explicitly learning the code functionalities. In contrast, 
% our approach to learn about program behavior is through contrastive reasoning. Since the model {\em explicitly} learns to reason about a code \wrt its functional equivalent and different counterparts during pretraining, our pretrained model outperforms other models even with a much smaller pretrained dataset. 

To this end, we carefully designed \tool's  pre-training to learn about syntactic and functional relationship between code components and 
% With the complicated and carefully design of our pre-training, we expect \tool to learn sufficient knowledge for downstream applications from limited amount of data and consequently save computing resources. 
We pre-train \tool on a \emph{small} dataset, with 865 MB of C code and 992 MB Java code from 100 most popular GitHub, and evaluate the model on code understanding and generation tasks: vulnerability detection, code clone detection and code summarization. Experiments show that our small models can outperform many baselines that are pre-trained on much larger datasets. Our analysis further illustrates that by adding carefully designed positive and negative code samples and the new NT-MLM objective, the model can better understand code during pre-training. The ablation study also reveals the potentials of pre-training our model with larger datasets and further improve the performance.

In summary, our major contributions are: 1) We design structure-guided code transformation heuristics to automatically augment traing data without human labels. We introduce {negative code samples} (carefully crafted to inject real-world bugs) for the first time, to better learn code contrasts. Our d bug injection strategy successfully encloses real-world security issues to the code. 2) We propose a new pre-training task, NT-MLM, to embed structural context to each token embedding. 3) We develop \tool, a self-supervised pre-training technique that can jointly and efficiently learn the textual, structural and functional properties of code. Even though pre-trained with significantly less data, \tool can match or outperform the state-of-the-art models on code understanding and generation tasks.


==> acl2022/body/3_data_augmentation.bck.tex <==
\section{Data Augmentation Without Human Labels}
\label{sec3:data_aug}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{iclr2022/figures/original_sample.png}
        \caption{Original Code}
        \label{fig:orig_sample}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{iclr2022/figures/positive_sample.png}
        \caption{Functionally Equivalent Code}
        \label{fig:pos_sample}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{iclr2022/figures/negative_sample.png}
        \caption{Bug Injected Code}
        \label{fig:neg_sample}
    \end{subfigure}
    
    % \caption{An example illustrating data augmentation. The original code is adapted from CVE-2021-38094 patch. With our automated code transformation, the original code is transformed to a functionality equivalent code by renaming and statements permutation, and the original code is also injected with a potential integer overflow bug. 
    % Considering overlapping tokens, \ref{fig:orig_sample} and \ref{fig:pos_sample} are significantly distinct even if they have the same functionality, while \ref{fig:orig_sample} shared most tokens with its buggy version \ref{fig:neg_sample}.
    \caption{An example illustrating data augmentation.~\ref{fig:orig_sample} shows the original code that is adapted from the CVE-2021-38094 patch. 
\ref{fig:pos_sample} shows functionality equivalent code of ~\ref{fig:orig_sample} where the original code is transformed by renaming and statements permutation. \ref{fig:neg_sample} shows a small variation from~\ref{fig:orig_sample} where a potential integer overflow bug is injected.}
\label{fig:data_aug}
\vspace{-5mm}
\end{figure}

% During pre-training, our goal is to train the model to identify the similar programs and differentiate the buggy programs from the benign ones. In order to do so, we need a labeled dataset to indicate the functionality and bugginess of each sample. Collecting such a dataset can be expensive and it is even more challenging if we expect the dataset to include enough data for pre-training. To this end, we design code transformation heuristics to automatically generate similar and buggy counterparts for a given code, so that the transformation can be applied to any amount of programs without human efforts. 
Goal of our pre-training is to train the model to identify the similar programs that can be structurally different (positive sample) and differentiate the buggy programs (negative sample) that share structural resemblances with the benign ones. Thus, for each original sample, we need a labeled positive and a negative example. Manually collecting such a dataset is expensive, especially at the scale of  pre-training. Here we design code transformation heuristics to automatically generate similar and buggy counterparts of a given code, so that the transformation can be applied to any amount of programs without human efforts. 

Given a code sample, we first parse the code into the AST.
% \lbc{do we create control/data flow? I thought treesitter can only build the ast} \scc{We do analyze the control and data dependencies while injecting noises.}
We analyze the AST and build a control/data flow graph from the AST. \rdc{should we say negative and then positive?}
We use this graph to apply our code transformation heuristics. 
For every original code sample ($x$), we apply semantic preserving transformation heuristics (\S\ref{subsec:similar_code_generation}) to generate a positive sample ($x^+$).
We also apply  bug injection heuristics (\S \ref{subsec:bug_injection}) to generate a hard-negative code example ($x^-$). 
We design the heuristics in a way that makes $x^+$ be the functional equivalent or semantic clone of $x$,  and $x^-$ be the buggy/noisy version of $x$. 
It is also worth noting that, not all heuristics are applicable to all code samples; we decide on applicable heuristic based on the flow graph of original code. 
% After that, we analyze the AST to identify the applicable heuristics and perform the code transformation to build a positive pair with similar functionality and a hard negative code pair with bugs.
Figure~\ref{fig:data_aug} shows 
% a real-world 
an
example of the code transformation. 
The code in figure \ref{fig:pos_sample} is the functional equivalent of figure \ref{fig:orig_sample}; even though they look drastically different. 
Figure \ref{fig:neg_sample} shows a buggy version of figure \ref{fig:orig_sample}, where the original code is injected with a potential integer-overflow bug and the expected behavior of the resultant code is unpredictable.  

% We can see that the majority of tokens for program \ref{fig:orig_sample} are different from \ref{fig:pos_sample} while preserving the functionality, but \ref{fig:orig_sample} shared most tokens with its buggy version.

\subsection{Bug Injection}
\label{subsec:bug_injection}

For generating hard negative sample ($x^-$) from a given code ($x$), we define six categories of bug injection heuristics. 
While generating such hard negative samples, our goal is to maintain maximum textual similarity of the original code, so that the model can learn to analyze source code beyond textual similarity. 
These heuristics are inspired by the buggy code patterns from a wide number of Common Weakness Enumeration (CWE) types (Appendix~\ref{appendix:bug_injection_cwe}). 
While it is very difficult to guarantee that $x^-$ will exhibit vulnerability or security bug, our heuristics will force $x^-$ to exhibit different functionality than $x$.

\textbf{Misuse of Data Type.}
Usage of a wrong data type can trigger several security flaws in the code. For instance, usage of a smaller data type (\eg~{\tt short}) in place of a larger one (\eg~{\tt long}) may result in overflow bug (\eg \citet{cve-2021-38094}). In addition, such errors are very difficult to track since these bugs are usually exhibited in input extremities (\ie very large or very small values), and for languages that support implicit type casting, such incorrect type may even cause imprecision bug -- resulting in the unpredictable behavior of the code. We intentionally change the data types inside $x$ with wrong ones to inject potential security bugs. 

\textbf{Misuse of Pointer.}
Incorrect use of pointers is a major concern of vulnerabilities in source code. Accessing an uninitialized pointer may lead to unpredictable behavior.
A {\tt NULL} pointer or already freed pointer could lead to Null Pointer Dereferencing vulnerability (\eg \citet{cve-2021-3449}). 
To inject pointer-related bugs, we randomly remove the initialization expression when a pointer is declared, or set some pointers to {\tt NULL}. 

\textbf{Change of Conditional Statements.}
Programmers usually check necessary preconditions using {\tt if-statement} before doing any safety critical operation. 
For instance, before accessing an array with an index, a programmer may add a condition checking the validity of the index. 
Lack of such checks can lead to buffer-overflow bug in code (\eg \citet{cve-2020-24020}). 
We observe that such checks surround very small lines of code ($\leq$ 5 lines). 
We introduce bug in the code by removing such small {\tt if-statement} statement. 
In addition, we also inject bug by modifying randomly selected arithmetic conditions. 
We replace the comparison operator ($<$, $>$, $\leq$, $\geq$, $==$, $!=$) with another operator, to inject potential out-of-bound access, forcing the program to deviate from its original behavior.

\textbf{Misuse of Variables.} 
When there are multiple variables present in a code scope (\eg a {\tt if} block surrounding number of statement), incorrect use of variables may lead to erroneous behavior of the program. 
Such errors are known as {\sc VarMisuse} bug~\citep{allamanis2018learning}. 
We induce code with such bugs by replacing a variable with another. 
To keep the resultant code compilable, we perform scope analysis on the AST and replace a variable with another variable reachable in the same scope. 

\textbf{Misuse of Values.}
Uninitialized variables, or variables with wrong values may alter the program behavior, may even cause security flaw (\eg ~\citet{cve-2019-12730}). We modify the original code by removing the initializer expression of variable. In addition, to induce the code with {\tt divide-by-zero} vulnerability, we identify the potential divisor variables from the flow graph and forcefully assign zero values to them immediately before the division. 

\textbf{Change of Function Calls.} We induce bug in the code by randomly changing arguments of function call. For a randomly selected function call, we add, remove, swap or assign {\tt NULL} value to arguments, forcing the code to behave unexpectedly. 

\subsection{Similar Code Generation}
\label{subsec:similar_code_generation}

In order to generate positive samples ($x^+$) from a given code, we use three different heuristics. 
In this case, our goal is to generate functionally equivalent code while inducing maximum textual difference. 
These heuristics are inspired by code clones~\citep{funaro2010hybrid, sheneamer2018detection}.


\textbf{Variable Renaming.}
Variable renaming is a typical code cloning strategy and frequently happens during software development~\citep{ain2019syscodeclone}. 
To generate such a variant of the original code, we either (a.) rename a variable in the code with a random identifier name or (b.) with an abstract name such as \texttt{VAR\_i}~\citep{roziere2021dobf}. 
While choosing random identifier names, we only select identifiers that are available in the dataset. 
For any variable renaming, we ensure that both the definition of the variable and subsequent usage(s) are renamed.
We also ensure that a name is not used to rename more than one variable. 

\textbf{Function Renaming.}
We rename function calls with abstract names like \texttt{FUNC\_i}. By doing this, we make more tokens different compared with the original code but keep the same syntax and semantics. We do not rename 
library calls for the code (\eg, \texttt{memcpy()} in C).

\textbf{Permutation of Statements.}
Relative order among the program statements that are independent of each other can be changed without altering the functionality of code.
More specifically, we focus on the variable declaration or initialization statements. 
We first conduct dependency analysis to identify a set of local variables that do not depend on other values for initialization. Then we move their declaration statements to the beginning of the function and permute them.
% \textbf{Motivation }
% %\rdc{Are we adding a figure to explain the tree operation?}
% %Detecting software bugs has always been significant to ensure software security, and nowadays, enormous amounts of open-source projects have become publicly available, making the task more challenging. 
% Researchers have explored the potentials of detecting security bugs with pre-trained models~\citep{feng2020codebert,guo2021graphcodebert,ahmad2021plbart,buratti2020cbert}. The existing models regard bug detection as a general code 
% % understanding 
% classification
% task while ignoring its characteristics. In some cases, the problematic function can look quite similar with its fixed version; they share most of the tokens and the overall tree structure, while only one or a few tokens trigger the bug behavior~\citep{ding2020patching}. 
% It will be hard to tell the difference between the buggy code and the patched code, if the model learns the former during training and comes across the latter during testing. 
% Our design of pre-training tends to teach the model about these bug patterns that are challenging to be detected but can cause unpredictable or even malicious code behaviors. 


% With these heuristics, our buggy counterparts can expose normal bugs and security issues covering many Common Weakness Enumeration (CWE) types (Appendix~\ref{appendix:bug_injection_cwe}) 
%and we successfully build hard negative samples~\citep{robinson2021hardnegative, gao2021simcse} of code \emph{without human-provided labels}. 

% \textbf{Misuse of Data Type.}
% Security bugs triggered by wrong types are common in programming languages like C and Java. For example, if we change a variable initialization with type \texttt{float} to \texttt{int}, a potential integer overflow is then injected (\eg \citet{cve-2021-38094}),
% \footnote{CVE-2021-38094 is triggered by type misuse: \url{https://github.com/FFmpeg/FFmpeg/commit/99f8d32129dd233d4eb2efa44678a0bc44869f23}},
% since \texttt{float} supports a wider value range than \texttt{int}. We replace types with others that have a smaller value range to inject security bugs.

%(e.g., \texttt{float} to \texttt{int}, \texttt{unsigned int} to \texttt{int}, \texttt{int64} to \texttt{int8}).

% \textbf{Misuse of Pointer.} \scc{Check this} The usage of pointers are significant for C and C++, and the misuse of pointers can lead to security issues
% (\eg \citet{cve-2021-3449})
%\footnote{CVE-2021-3449 is triggered by null pointers: \url{https://git.openssl.org/gitweb/?p=openssl.git;a=commitdiff;h=fb9fa6b51defd48157eeb207f52181f735d96148}}
% such as null pointer dereference (\eg \citet{cve-2021-3449}) or access of unitialized pointers. We inject pointer-related bugs by changing a normal pointer to be null or uninitialized.


% A common fix for security bugs like out-of-array access and buffer overflow is to add if-statement as a security check to ensure the accessing element is in the scope of an array or buffer (\eg \citet{cve-2020-24020})
% %\footnote{CVE-2020-24020 is fixed by adding overflow checks: \url{https://github.com/FFmpeg/FFmpeg/commit/584f396132aa19d21bb1e38ad9a5d428869290cb}}. 
% From our observation, such security checks are always small ($\leq$ 5 lines) \texttt{if-statement}, since most checks are straightforward. We reverse this bug fixing process to introduce the flaw. We remove small \texttt{if-statement} from original code to change its functionality.

% \textbf{Wrong Equality Operators } We modify the equality operators including $<$, $>$, $\leq$, $\geq$, $==$, $!=$. Considering a statement is to check whether the index is strictly smaller than the array's size, we can replace $<$ to $\leq$ to allow a potential out-of-array access.

% {\bf Change of Conditional Statements.} In addition to 

% \textbf{Abnormal Variable } 1) Uninitialized variable. In C and C++, stack variables are not initialized by default, so uninitialized variables can be hacked (\eg ~\citet{cve-2019-12730}). We remove the initialized value of some variables to inject such a bug. 2) Wrong Value. We change the variable's value to an unexpected one. For example, we identify the variables that can potentially be divisors and assign them a value of zero before the division, to trigger divide-by-zero vulnerability; and we replace boolean value with its opposite value. 3) Variable misuse. We borrow the idea from \citet{allamanis2018learning} that some variables are used by mistake at certain places. To inject bug, we randomly replace variables in the original code with other identifier names in the scope.

% \textbf{Abnormal Function Calls } We modify the function arguments: we swap, remove or assign a \texttt{NULL} value to the callee's argument list. By doing this, we can trigger unexpected behaviors of the callee including type misuse, pointer misuse and abnormal variable.


% \subsection{Similar Code Generation}
% \label{subsec:similar_code_generation}

% \textbf{Motivation } Identifying similar code snippets from large codebases has always been challenging yet significant for software evolution and maintenance~\citep{kim2017vuddy, ain2019syscodeclone}. For instance, if a vulnerability is reported in a system, all its copies or clones should be carefully checked to ensure software security, and accurately detecting these similar code snippets is a prerequisite. 
% %While existing pre-trained token embeddings keep playing an important role in revealing code semantics for similarity detection~\citep{feng2020codebert,guo2021graphcodebert,ahmad2021plbart}, 
% We observe that the functional similarity of programs is not necessarily proportional to the token or syntax similarity. Semantic code clones (e.g., two distinct implementations of quicksort algorithm) can share very few tokens but perform the same functionality. Therefore, token or syntax-based pre-training cannot provide enough knowledge to identify the functionality similarity. Our work intends to empower the model with a sense of code similarity not only based on tokens and syntax, so we generate semantically equivalent counterparts for each sample. 
% %We consider three main strategies to transform the code to its similar clone.

% \textbf{Variable Renaming }
% Variable renaming is a typical code clone strategy and frequently happens during software development~\citep{ain2019syscodeclone}. To generate a similar code clone, given a source code file, we will 1) rename all variables in the scope with a randomly selected set of "real" variable names in our dataset, or 2) with an abstract name such as \texttt{VAR\_i}~\citep{roziere2021dobf}. These two strategies will be chosen randomly for renaming. Noted that our renaming strategy will only change the textual information while preserving the syntax and semantics of the original code.

% \textbf{Function Call Renaming }
% We rename function calls with abstract names like \texttt{FUNC\_i}. By doing this, we make more tokens different compared with the original code but keep the same syntax and semantics. We do not rename the 
% % built-in 
% library call for the code (\eg, \texttt{memcpy()} in C).

% \textbf{Permutation of statements }
% We permute the statements while keeping the semantics. Specifically, we focus on the statements of variable declarations and initialization inside a function. We first conduct dependency analysis to identify a set of local variables that do not need other variable's value for initialization. Then we move their initialization or declaration statements to the beginning of the function and permute them.

%To conclude, given a code sample, we will first identify the applicable heuristics, and apply all of them to transform the code to build a positive pair with similar functionality and a hard negative code pair with bugs. All the steps are completely automated, and we can apply the code transformation to very large dataset with acceptable time cost without human efforts.


==> acl2022/body/4_model.bck.tex <==
\section{\tool}
\label{sec4:model}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{iclr2022/figures/model-overview.png}
    \caption{An illustration of \tool pre-training with a minibatch of three. The original code and its node types will be randomly masked with $[MASK]$, and the final representation of masked tokens will be used to recover their source tokens and node types. The original code, say $x$, will also be transformed to build ($x, x^+, x^-$). Then the pair will be fed into the \textbf{same} transformer encoder and get the embedding of each sequence with $[CLS]$ tokens for contrastive learning.}
    \label{fig:model_arch}
    \vspace{-5mm}
\end{figure}

This section presents the model architecture, input representation and pre-training tasks.
\tool uses a 12-layered transformer encoder~\citep{vaswani2017transformer} model similar to BERT~\citep{devlin-etal-2019-bert}.
We feed the model with both textual information from the source code and structural information from the syntax tree (\S\ref{subsec:input_repr}). 
We pretrain \tool using three different pretraining tasks (\S\ref{subsec:pretraining-task}). 
Figure \ref{fig:model_arch} depicts an example workflow of \tool. 
%We first transform the code to a positive and a negative counterparts, with automated code transformation algorithms (\S\ref{sec3:data_aug}). Then 
We randomly select tokens in the original sample and mask them and their node types, and then use the embedding of these masks to predict them back. We further extract the sequence embeddings within a minibatch and learn to contrast them based on the code functionality. 

\subsection{Input Representation}
\label{subsec:input_repr}
\textbf{Source Code.} Given a program ($x$), we apply a lexical analyzer to tokenize it based on the language grammar and flatten the program as a token sequence ($x_1 x_2 ... x_m$, where $x_i$ is i'th token in the code).
We further train a sentencepiece~\citep{kudo-richardson-2018-sentencepiece} tokenizer based on such flattened code token sequences with vocabulary size 20,000. 
We use this tokenizer to divide the source code tokens into subtokens. 
We prepend the subtoken sequence with a special token {\tt [CLS]} and append with a special token {\tt [SEP]}. 
Finally, \tool converts the pre-processed code sequence $C = \{[CLS], c_1, c_2, ..., c_k, [SEP]\}$ to vectors $V^{src} = \{v_{[CLS]}^{src}, v_1^{src}, v_2^{src}, ..., v_k^{src}, v_{[SEP]}^{src}\}$ with a token embedding layer.

\textbf{AST Node Types.} 
For every token in input code, we extract the node type ($tt$) from the syntax tree. 
Since such types are all terminal node types (\eg keyword, identifier, punctuation), we do not get enough information about the structure only with these types. 
In order to add more information about the tree, for each token, we also extract its parent type ($pt$). 
Such parent type provides us with information about the context of a token. 
For instance, when parent type of an {\tt idenfier} is {\tt Function-Declarator}, we know that that identifier is a function name. 
In contrast, when the {\tt identifier}'s parent is a {\tt Binary Expression}, it should a variable.
Consequently, we annotate each code sub-token $c_i$ with a type token $t = tt\#pt$. 
It is worth noting that, subtokens coming from the same original code token will all have the same type. 
Therefore, we have the node type sequence for the code $T = \{[CLS], t_1, t_2, ..., t_k, [SEP]\}$, and \tool converts it as vectors $V^{type} = \{v_{[CLS]}^{type}, v_1^{type}, v_2^{type}, ..., v_k^{type}, v_{[SEP]}^{type}\}$ with a type embedding layer.
Appendix Table~\ref{tab: node_type} shows an example of code tokens and their node types.
\tool generates token representation $v_i$ of subtoken $c_i$ as a sum of token embedding $v_i^{src}$ and type embedding $v_i^{type}$.

\subsection{Pre-training}
\label{subsec:pretraining-task}
Our aim for pretraining \tool is to train the model to learn robust representation of the source code. We aim training the \tool to learn representation of source code based on (a.) textual context, (b.) syntax tree, and (c.) code functionality. In that spirit, pretrain \tool to optimize on three different objectives, \ie Masked Language Model (MLM), Node Type - Masked Language Model (NT-MLM) and Contrastive Learning (CLR).

For a given code $x$, we first embed the tokens and node-types to vectors $V = \{v_{[CLS]}, v_1, ..., v_{[SEP]}\}$. We optimize MLM loss ($\mathcal{L}_{MLM}$) (\S\ref{subsec:mlm}) and NT-MLM loss ($\mathcal{L}_{NT-MLM}$) (\S\ref{subsec:ntmlm}) based on $x$. These two loss functions learn about the textual and syntactic context of source code. For every code $x$ in a minibatch of input, we generate positive example $x^+$ and hard-negative example $x^-$ using the heuristics described in Section \ref{sec3:data_aug}. We optimize CLR loss ( $\mathcal{L}_{CLR}$) (\S\ref{subsec:clr}) on original code and its positive and hard-negative counterparts. 
The final loss function to optimize for pretraining \tool is 
\begin{equation}
    \mathcal{L}(\theta) = \mathcal{L}_{MLM}(\theta) + \mathcal{L}_{NT-MLM}(\theta) + \mathcal{L}_{CLR}(\theta)
\end{equation}
%\begin{equation}
%    \mathcal{L}(\theta) = \alpha * \mathcal{L}_{MLM}(\theta) + \beta * \mathcal{L}_{NT-MLM}(\theta) + \gamma * \mathcal{L}_{CLR}(\theta)
%\end{equation}
%Where, $\alpha$, $\beta$, and $\gamma$ are empirically set hyperparameters. 
%\rdc{I do not want to highlight such hyperparameters, since we did not do sufficient discussions on that.} \scc{But not all the losses carry equal weight, right?} \rdc{No, but we only try different weight for NT-MLM.}

% \tool pretrains its transformer model with takes $V = \{v_{[CLS]}, v_1, ..., v_{[SEP]}\}$, which contains both the textual and syntactic information of code samples, as input. Then we take the output of the last layer of the transformer encoder $H = \{h_{[CLS]}, h_1, ..., h_{[SEP]}\}$ for the following three pre-training tasks. 

\subsubsection{Masked Language Model}
\label{subsec:mlm}
% As shown in Figure~\ref{fig:model_arch}, 
We apply the standard masked language model to the original code ($x$). Given a source code sequence $C$, we randomly choose 15\% of tokens and replace them with a special token $[MASK]$ for 80\% of the time and a random token for 10\% of the time and leave the rest 10\% unchanged. We record the indices of masked token as $loc_m$, replaced token as $loc_r$ and unchanged tokens as $loc_u$ for node-type MLM. We define the union of these indices as $M = loc_m \cup loc_r \cup loc_u$. MLM will learn to recover the masked source code $\{c_i | i \in M\}$ given the transformer encoder's output $h_i$. We present the loss for MLM as 
$\mathcal{L}_{MLM} = \sum_{i \in M} - log P(c_i | h_i)$
%\begin{equation}
%    \mathcal{L}_{MLM} = \sum_{i \in M} - log P(c_i | h_i)
%\end{equation}
%\lbc{same of NODE TYPE MLM}
\subsubsection{Node-type Masked Language Model } 
\label{subsec:ntmlm}
%\lbc{are we sure it's clear what a node-type is? Fig 2 does not fully explain this. maybe we should provide an example}
Token-based MLM re-builds the token using its surrounding tokens and successfully encodes the contextual information into each token representation. Motivated by MLM, we propose the tree-based context-aware pre-training task, to encode the structural context, such as parent, sibling and children nodes. As we shown in Figure~\ref{fig:model_arch}, we flatten the ASTs as sequences and we expect the flattened trees can well preserve the local structure information (i.e., sub-trees containing terminal nodes), and existing work~\citep{Chakraborty2020codit} has empirically shown such potentials. To this end, we introduce node-type masked language model (NT-MLM). Given the corresponding node type sequence $T$ of source code $C$, we mask the node types $\{t_p | p \in loc_m\}$ with the special token $[MASK]$, and replace the node types $\{t_q | q \in loc_r\}$ with random tokens. Specifically, by doing this, we make sure that if a source code token is chosen to be masked or replaced, its corresponding node type will be performed the same operation. NT-MLM will learn to recover the masked source code $\{t_i | i \in M\}$ given the transformer encoder's output $h_i$. We present the loss for NT-MLM as 
$\mathcal{L}_{NT-MLM} = \sum_{i \in M} - log P(t_i | h_i)$
%\begin{equation}
%    \mathcal{L}_{NT-MLM} = \sum_{i \in M} - log P(t_i | h_i)
%\end{equation}
%\lbc{why this equation does not have its own section like for LCLR}

\subsubsection{Contrastive Learning } 
\label{subsec:clr}
We adopt contrastive learning to focus on the functional characteristics of code. With the structure-guided code transformation algorithms in Section~\ref{sec3:data_aug}, we are able to generate a positive sample ($x^+$ in Figure~\ref{fig:model_arch}) and a hard negative sample ($x^-$ in Figure~\ref{fig:model_arch}) for each program in the dataset. 
More specifically, we have a minibatch of $N$ programs, and for each program, we extract the sequence representation from the transformer outputs $\mathbf{h} = h_{[CLS]}$. We will augment every sequence in the minibatch with positive and negative samples, and then the minibatch is extended to N pairs of $(\mathbf{h}, \mathbf{h}^+, \mathbf{h}^-)$. We refer to the contrastive loss with hard negative samples from \citet{gao2021simcse} and we adapt it to our scope as follows. We use cosine similarity as the $sim()$ function and $\tau$ is the temperature parameter to scale the loss, and we use $\tau = 0.05$. 
\begin{equation}
    \mathcal{L}_{CLR} = -\log\frac{\mathbf{e}^{\text{sim}\left(\mathbf{h}, \mathbf{h}^+\right)/\tau}}{\sum^{N}_{n=1}\left(\mathbf{e}^{\text{sim}\left(\mathbf{h}, \mathbf{h}_{n}^+\right)/\tau} + \mathbf{e}^{\text{sim}\left(\mathbf{h}, \mathbf{h}_{n}^-\right)/\tau} \right)}
\end{equation}

%To conclude, the model will be pre-trained with three tasks to learn the textual, syntactical and functional properties of code. The final loss function is given below, where $\theta$ contains all trainable weights of the model. We optimize the model by minimize this final loss.
%\begin{equation}
%    \mathcal{L}(\theta) = \mathcal{L}_{MLM}(\theta) + \mathcal{L}_{NT-MLM}(\theta) + \mathcal{L}_{CLR}(\theta)
%\end{equation}





% This section presents the model architecture and pre-training tasks. We follow the design of BERT~\citep{devlin-etal-2019-bert}, using a stack of transformers encoders to build the pre-training model. As shown in Figure~\ref{fig:model_arch}, we train the model with three tasks jointly: Masked Language Model (\S\ref{subsec:mlm}), Node Type - Masked Language Model (\S\ref{subsec:ntmlm}) and Contrastive Learning (\S\ref{subsec:clr}). We consider two modalities of code information as the model input, source code and AST node types, to include the textual and syntactic information of code.

% \subsection{Textual and Structural Input } 
% \label{subsec: model_input}


% \textbf{Source Code.}
% Given a program, we will firstly apply a lexical analyzer to tokenize it based on the language grammar and flatten the program as a token sequence. To avoid the unlimited vocabulary problem in source code modeling~\citep{hellendoorn2017aredeepneural, karampatsis2020bigcode}, we train sentencepiece~\citep{kudo-richardson-2018-sentencepiece} to learn a 20,000 subword vocabulary and split the code tokens into sub-tokens. Then we follow the input design of \citet{devlin-etal-2019-bert} that we add special tokens to the pre-processed code sequence $C = \{[CLS], c_1, c_2, ..., c_k, [SEP]\}$ . \tool will convert the source code sequence as vectors $V^{src} = \{v_{[CLS]}^{src}, v_1^{src}, v_2^{src}, ..., v_k^{src}, v_{[SEP]}^{src}\}$.

% \textbf{AST Node Types.} To get the structure information, we parse the source code into an AST. We use all the source code tokens generated by the lexical analyzer as the terminal node and build AST on them. The lexical analyzer will also assign each token a type $tt$ (e.g., keyword, identifier, punctuation) and we use such a type as the terminal node type. With AST, we will also locate the parent node for each terminal node, which contains the local sub-tree information. We observe that the type of the parent node, $pt$, can well encode such local structures, so for each terminal node, we give it a type by combining its own type and the parent type with "\#", i.e., node type $t = tt\#pt$. So far, we assign a node type for each source code token to indicate its local structure information. Noted that all sub-tokens splited by the same token will share the token type. Therefore, we have the node type sequence for the code $T = \{[CLS], t_1, t_2, ..., t_k, [SEP]\}$, and \tool will convert it as vectors $V^{type} = \{v_{[CLS]}^{type}, v_1^{type}, v_2^{type}, ..., v_k^{type}, v_{[SEP]}^{type}\}$.
% Appendix Table~\ref{tab: node_type} shows an example of code tokens and their node types. 

% Having the textual representation $v_i^{src}$ and the structural representation $v_i^{type}$, we further aggregate them as the final model input, $v_i = Aggr(v_i^{src}, v_i^{type})$. We will use $sum$ as our main aggregation method.


% \subsection{Pre-training}
% \label{subsec:pretraining-task}
% \tool takes $V = \{v_{[CLS]}, v_1, ..., v_{[SEP]}\}$, which contains both the textual and syntactic information of code samples, as input. Then we take the output of the last layer of the transformer encoder $H = \{h_{[CLS]}, h_1, ..., h_{[SEP]}\}$ for the following three pre-training tasks. 

% \subsubsection{Masked Language Model}
% \label{subsec:mlm}
% As shown in Figure~\ref{fig:model_arch}, we apply the standard masked language to the original code. Given a source code sequence $C$, we randomly choose 15\% of tokens and replace them with a special token $[MASK]$ for 80\% of the time and a random token for 10\% of the time and leave the rest 10\% unchanged. We record the indices of masked token as $loc_m$, replaced token as $loc_r$ and unchanged tokens as $loc_u$ for node-type MLM. We define the union of these indices as $M = loc_m \cup loc_r \cup loc_u$. MLM will learn to recover the masked source code $\{c_i | i \in M\}$ given the transformer encoder's output $h_i$. We present the loss for MLM as 
% %$\mathcal{L}_{MLM} = \sum_{i \in M} - log P(c_i | h_i)$

% \begin{equation}
%     \mathcal{L}_{MLM} = \sum_{i \in M} - log P(c_i | h_i)
% \end{equation}

% \subsubsection{Node-type Masked Language Model } 
% \label{subsec:ntmlm}
% Token-based MLM re-builds the token using its surrounding tokens and successfully encode the contextual information into each token representation. Motivated by MLM, we propose the tree-based context-aware pre-training task, to encode the structural context, such as parent, sibling and children nodes. As we shown in Figure~\ref{fig:model_arch}, we flatten the ASTs as sequences and we expect the flattened trees can well preserve the local structure information (i.e., sub-trees containing terminal nodes), and existing work~\citep{Chakraborty2020codit} has empirically shown such potentials. To this end, we introduce node-type masked language model (NT-MLM). Given the corresponding node type sequence $T$ of source code $C$, we mask the node types $\{t_p | p \in loc_{mask}\}$ with the special token $[MASK]$, and replace the node types $\{t_q | q \in loc_{rep}\}$ with random tokens. Specifically, by doing this, we make sure that if a source code token is chosen to be masked or replaced, its corresponding node type will be performed the same operation. NT-MLM will learn to recover the masked source code $\{t_i | i \in M\}$ given the transformer encoder's output $h_i$. We present the loss for NT-MLM as follows
% \begin{equation}
%     \mathcal{L}_{NT-MLM} = \sum_{i \in M} - log P(t_i | h_i)
% \end{equation}


% \subsubsection{Contrastive Learning } 
% \label{subsec:clr}
% %With sufficient knowledge about code text and syntax, the model can still struggle to identify the code functionality, since two programs can be very different in terms of text and syntax while sharing the same functionality (explained in Section~\ref{subsec:similar_code_generation}), but an abnormal program can share the tree structure and most tokens with the normal one (explained in Section~\ref{subsec:bug_injection}). Therefore, 
% We adopt contrastive learning to focus on the functional characteristics of code. With the structure-guided code transformation algorithms in Section~\ref{sec3:data_aug}, we are able to generate a positive sample ($x^+$ in Figure~\ref{fig:model_arch}) and a hard negative sample ($x^-$ in Figure~\ref{fig:model_arch}) for each program in the dataset. Formally, say we have a minibatch of N programs, and for each program, we extract the sequence representation from the transformer outputs $\mathbf{h} = h_{[CLS]}$. With the automated code transformation, we will augment the minibatch with positive and negative samples, and then the minibatch is extended to N pairs of $(\mathbf{h}, \mathbf{h}^+, \mathbf{h}^-)$. We refer to the contrastive loss with hard negative samples from \citet{gao2021simcse} and we adapt it to our scope as follows. We use cosine similarity as the $sim()$ function and $\tau$ is the temperature parameter to scale the loss, and we use $\tau = 0.05$.
% \begin{equation}
%     \mathcal{L}_{CLR} = -\log\frac{\mathbf{e}^{\text{sim}\left(\mathbf{h}, \mathbf{h}^+\right)/\tau}}{\sum^{N}_{n=1}\left(\mathbf{e}^{\text{sim}\left(\mathbf{h}, \mathbf{h}_{n}^+\right)/\tau} + \mathbf{e}^{\text{sim}\left(\mathbf{h}, \mathbf{h}_{n}^-\right)/\tau} \right)}
% \end{equation}

% To conclude, the model will be pre-trained with three tasks to learn the textual, syntactical and functional properties of code. The final loss function is given below, where $\theta$ contains all trainable weights of the model. We optimize the model by minimize this final loss.
% \begin{equation}
%     \mathcal{L}(\theta) = \mathcal{L}_{MLM}(\theta) + \mathcal{L}_{NT-MLM}(\theta) + \mathcal{L}_{CLR}(\theta)
% \end{equation}





==> acl2022/body/6_analysis.tex <==
\section{Analysis}
\label{sec6:analysis}
\begin{wrapfigure}{r}{0.4\linewidth}
    \begin{center}
    \includegraphics[width=0.4\columnwidth]{acl2022/figures/ppl.png}
    \end{center}
    \caption{\small The evaluation perplexity of last five epochs for different \tool variations.}
    \label{fig:ppl}
    \vspace{-3mm}
\end{wrapfigure}
\textbf{Impacts of Augmented Samples and NT-MLM.} Language model perplexity is an important metric to evaluate the quality of pre-trained embeddings. To better understand how data augmentation and NT-MLM objective affect the pre-training quality, we keep evaluating the perplexity of \tool's three variations (Section~\ref{subsec:expr_pretrain}) on the held-out data during pre-training. 


We plot the last five epochs in Figure~\ref{fig:ppl}. As we explained in Figure~\ref{fig:model_arch}, we only apply MLM to the original sample $x$ regardless of the existence of $(x^+, x^-)$, so it is fair to compare among three models. We can see that the model with hard negative samples keeps having lower perplexity than \mlmclr model, and the model with node type information has even lower perplexity than both models that only consider source code tokens. This indicates that even if the models always come across the same sequences for MLM, learning the contrast of the hard negative pairs with tree-based context can further help the model understand the sequence.



%\textbf{Impacts of Augmented Samples and NT-MLM } Language model perplexity is an important metric to evaluate the quality of pre-trained embeddings. To better understand how data augmentation and NT-MLM objective affect the pre-training quality, we keepplot the perplexity of \tool's three variations (Section~\ref{subsec:expr_pretrain}) during the pre-training, using the held-out split of our dataset. As we explained in Figure~\ref{fig:model_arch}, we only apply MLM to the original sample $x$ regardless of the existence of $(x^+, x^-)$, so all three variations will gain the same knowledge only through MLM. Interestingly, as shown in Figure~\ref{fig:ppl}, we can see that the model with hard negative samples keeps having lower perplexity than MLM+CLR model. This indicates that even if the models always come across the sequences for MLM, learning the contrast of the hard negative pairs can further help the model understand the sequence. Also, the model with node type information has even lower perplexity than both models that only consider source code tokens. This result empirically reveal that the context including node-type information can further help the model restrict the search space for picking up the correct missing token. This figure, in fact, provide strong evidence that all three objectives of our model are aligned well and can be optimized together to help the model better understand the textual, structural and functional aspects of code. 
\input{acl2022/tables/medium_model}
\textbf{Medium Pre-trained Model }
As shown in Section~\ref{sec5:expr}, \tool trained on a small dataset achieves comparable or even better performance than models pre-trained on large datasets in code understanding and generation tasks (Let's call this version  \toolS). We further explore the benefits of pre-training using larger data. We pre-train a {\sc Medium} model, \toolM,  on our extended datasets with top-10,000 C-language Github repositories (13G). We evaluate \toolM on C-language tasks. The results are shown in Table~\ref{tab: medium_model}. Increasing the pre-training dataset improves the performance of downstream tasks. Note that our medium dataset is still smaller than the large dataset of the baseline models (13G vs.~20G).  
%In the future, we will further augment our pre-training dataset with top-10,000 Java Github repositories and try on Java downstream tasks.



%\textbf{Textual and Structural Representation Aggregation } \rdc{Maybe go to appendix.}


==> acl2022/tables/bigclonebench_result.tex <==
\begin{wraptable}{R}{0.43\textwidth}
%\begin{table}
\caption{\small Results of BigCloneBench for code clone detection}
\label{tab:poj_result}
\scriptsize
\begin{tabular}{lrrr}\hline
Model &Prec. &Rec. & F1 \\\hline
CodeBERT$^*$ &94.7 &93.4 &94.1 \\
GraphCodeBERT$^*$ &94.8 &95.2 &95.0 \\\hline
\tool & \\
MLM + CLR &93.2 &93.9 &93.5 \\
MLM + CLR\_HN &N/A &N/A &N/A \\
MLM + CLR\_HN + NT-MLM &N/A &N/A &94.2 \\
\hline
\end{tabular}

\begin{flushleft}
\scriptsize 
*The authors of both works fixed bugs in their evaluation tool and updated the results in their Github repositories. We take the latest results for comparison.
\end{flushleft}
\vspace{-2mm}
\end{wraptable}

==> acl2022/tables/bug_injection.tex <==
\begin{table}
\caption{Bug injection operations.}
\label{tab: bug_injection_details}
\small
\begin{tabular}{lrr}\hline
Category &BLEU-4 \\\hline
Seq2Seq &15.09 \\
Transformer &16.26 \\
Roberta (code) &16.47 \\
CodeBERT &17.65 \\ \hline
\tool & \\
MLM+CLR &\textbf{17.89} \\
MLM+CLR\_HN &17.76 \\
MLM+CLR\_HN+NT-MLM &17.78 \\
\hline
\end{tabular} 
\vspace{-2mm}
\end{table}

==> acl2022/tables/code_summarization.tex <==
%\begin{wraptable}{R}{0.38\textwidth}
%\begin{table}
\begin{table}[ht]\centering
\caption{Result of code summarization}
\label{tab: code_summarization}

\small
\begin{tabular}{lrr}\hline
Model &BLEU-4 \\\hline
Seq2Seq &15.09 \\
Transformer &16.26 \\
Roberta (code) &16.47 \\
CodeBERT &17.65 \\ \hline
\tool & \\
\mlmclr &\textbf{17.89} \\
\mlmclrpn &17.76 \\
\tmlmclrpn &17.78 \\
\hline
\end{tabular} 

\vspace{-4mm}
\end{table}
%\end{wraptable}

==> acl2022/tables/dataset.tex <==
\begin{table}[h]
\caption{Pre-training dataset size}
\small
%\begin{minipage}{\linewidth}
\begin{center}
\begin{tabular}{|l|c|c|c|}
%\begin{adjustbox}{max width=\linewidth}
\hline
%                   & \textbf{# of Repositories} & \textbf{Size} & \textbf{Duplicates} \\
\textbf{Dataset} & \textbf{Repositories Count}             &   \textbf{Files Count} & \textbf{Total Size}\\
 \hline
Java {\sc small} & 100 & 187,214 & 992M \\
%\midrule
C {\sc small}  & 100 & 64,340 & 865M \\
%\midrule
Java {\sc large} & 10,000 & 3,292,777 & 13G \\%4,401,062 & 1,108,285 \\
%/midrule
C {\sc large} & 10,000 & 860,618 & 12G \\%4,079,552 & 3,218,934 \\
%\midrule
%\midrule
\hline
%\end{adjustbox}
\end{tabular}
\end{center}

\label{tab: pre-train-stats}
\end{table}

==> acl2022/tables/poj104_result.tex <==

\begin{wraptable}{R}{0.43\textwidth}
%\begin{table}
\caption{Results of POJ-104 for code clone detection}
\label{tab:poj_result}
\scriptsize
\begin{tabular}{lrr}\hline
Model &MAP@R \\\hline
Transformer &62.11 \\
RoBERTa (code) &76.67 \\
MISIM-GNN &82.45 \\
CodeBERT &82.67 \\\hline
\tool & \\
MLM + CLR &82.44 \\
MLM + CLR\_HN &82.73 \\
MLM + CLR\_HN + NT-MLM &\textbf{82.77} \\
\hline
\end{tabular}
\vspace{-2mm}
%\end{table}
\end{wraptable}

==> removed_text.tex <==
%abstract

Large pre-trained BERT models were originally introduced to process natural languages (NL) and have recently reported promising performance for understanding programming languages (PL). 
However, the initial success of the transplanted BERT model does not necessarily mean it is well-designed for PL. 
Masked Language Model (MLM) is the most frequently used objective for pre-training due to its compelling power to learn token embeddings. 
Nevertheless, the MLM objective itself is not enough to fully comprehend PL. PL maintains a more restricted structure (e.g., abstract syntax tree) with the corresponding grammar, and token-based MLM will struggle to capture such information. 
Additionally, even with excellent token representations, the model can still get confused when trying to understand code semantics: two programs can contain very different tokens but share the same functionality, but if we do minor changes (e.g., replace $<$ with $\leq$) to a code snippet, its behavior can be unpredictable and even trigger security bugs. 

% dataset

%The pre-training corpus is collected by downloading open source C and Java repositories from  GitHub. 
%In order to have good quality source code, we sort the repositories by the number of stars, with the top ranked repository having the most stars. 
%We then download the first 100 top ranked repositories for each of the Java and C {\sc small} datasets, and the first 10,000 top ranked repositories for each of the Java and C {\sc large} datasets. 
%As a further quality check, we excluded forks to avoid duplicates and we also filtered out repositories for which the readme is not primarily in English. 
%To further alleviate the problem of duplicate code, we applied deduplication on the {\sc large} dataset, as indicated by ~\citep{allamanis-deduplication}. 
%To avoid duplicate code, we excluded forks and applied deduplication in the {\sc large} datasets, as indicated by~\citep{allamanis-deduplication}.
%We did not perform deduplication for the {\sc small} datasets.
%During manual inspection we observed that many of the top ranked repositories had print statements which were hundreds of lines long and not in English. 
%Such repositories were excluded simply by checking to see if the readme was primarily in English and filtering out those that were not.
%We only consider the ".java" and ".c" files for Java and C repositories respectively. 
%Source code is kept as is, the only pre-processing we do is the removal of comments and empty lines. 
%All the selected source files are put together and then divided randomly to create training, validation and test sets using 95\%, 4\%, 1\% of the files respectively. 
%Details about the respository count, file count and total size of each dataset can be found in table \ref{tab: pre-train-stats}. 
%Java and C datasets are roughly the same size, despite the huge disparity in the number of files.


Corder~\citep{bui2021corder} represents programs as ASTs and apply contrastive learning. They reported their best results on POJ-104 with a model pre-trained with 1,000 Github repositories, while we use 100. Compared with them, \tool uses standard MLM to capture the textual information and AST node types to encode local tree structures while they directly map an AST to the vector space, and we introduce buggy contrasts to improve the difficulty of contrastive learning. 
